Making Deep Neural Networks Robust to Label Noise: a Loss Correction Approach

We present a theoretically grounded approach to train deep neural networks, including recurrent networks, subject to class-dependent label noise. We propose two procedures for loss correction that are agnostic to both application domain and network architecture. They simply amount to at most a matrix inversion and multiplication, provided that we know the probability of each class being corrupted into another. We further show how one can estimate these probabilities, adapting a recent technique for noise estimation to the multi-class setting, and thus providing an end-to-end framework. Extensive experiments on MNIST, IMDB, CIFAR-10, CIFAR-100 and a large scale dataset of clothing images employing a diversity of architectures --- stacking dense, convolutional, pooling, dropout, batch normalization, word embedding, LSTM and residual layers --- demonstrate the noise robustness of our proposals. Incidentally, we also prove that, when ReLU is the only non-linearity, the loss curvature is immune to class-dependent label noise.

==> big_table.tex <==
% This is a backup of the big table before touching results


\begin{table*}
\tiny
\centering
\begin{tabular}{|l|c|c|c|c|c|}
\toprule
\multicolumn{6}{c}{MNIST, fully connected} \\
\midrule
 & \textsc{no noise}& \textsc{mild symm.} & \textsc{high symm.} & \textsc{mild asymm.} & \textsc{high asymm.} \\
 & & $N=0.2$ & $N=0.6$ & $N=0.2$ &  $N=0.6$ \\
\midrule
 \hline
 cross-entropy &      $97.9 \pm 0.0$ & $\bm{96.9 \pm 0.1}$ & $93.9 \pm 0.3$ & $97.5 \pm 0.0$ & $53.0 \pm 0.6$  \\
 \hline
       backward  &      $97.9 \pm 0.0$ & $96.3 \pm 0.1$ & $92.6 \pm 0.2$ & $96.6 \pm 1.1$ & $\bm{93.0 \pm 0.9}$  \\
       backward $\hat{T}$  &      $97.9 \pm 0.0$ & $\bm{96.9 \pm 0.0}$ & $90.0 \pm 0.3$ & $96.7 \pm 0.1$ & $67.4 \pm 1.5$  \\
       forward  &      $97.9 \pm 0.0$ & $\bm{97.3 \pm 0.0}$ & $\bm{95.2 \pm 0.3}$ & $\bm{97.7 \pm 0.0}$ & $\bm{97.3 \pm 0.0}$  \\
       forward $\hat{T}$  &      $97.9 \pm 0.0$ & $\bm{96.9 \pm 0.0}$ & $93.8 \pm 0.3$ & $\bm{97.7 \pm 0.0}$ & $64.9 \pm 4.4$  \\
 \hline
       unhinged (BN) &     $97.6 \pm 0.0$ & $\bm{96.9 \pm 0.1}$ & $91.3 \pm 0.3$ & $97.0 \pm 0.1$ & $\bm{71.2 \pm 1.0}$  \\
       sigmoid (BN) &      $97.2 \pm 0.1$ & $93.1 \pm 0.2$ & $78.5 \pm 1.0$ & $96.7 \pm 0.1$ & $\bm{71.4 \pm 1.3}$ \\
       savage  &      $97.3 \pm 0.0$ & $\bm{96.9 \pm 0.0}$ & $\bm{95.0 \pm 0.1}$ & $97.0 \pm 0.1$ & $51.3 \pm 0.4$  \\
       bootstrap soft  &      $97.9 \pm 0.0$ & $\bm{96.9 \pm 0.0}$ & $94.0 \pm 0.1$ & $97.5 \pm 0.0$ & $53.0 \pm 0.4$  \\
       bootstrap hard  &      $97.9 \pm 0.0$ & $96.8 \pm 0.0$ & $93.8 \pm 0.2$ & $97.4 \pm 0.0$ & $55.0 \pm 1.3$  \\
\midrule       
\multicolumn{6}{c}{IMDB, word embedding} \\
\midrule
 & \textsc{no noise}& \textsc{mild symm.} & \textsc{high symm.} & \textsc{mild asymm.} & \textsc{high asymm.} \\
 & & $N=0.1$ & $N=0.4$ & $N=0.1$ &  $N=0.4$ \\
\midrule
 \hline
 cross-entropy &      $86.7 \pm 0.0$ & $84.6 \pm 0.1$ & $52.6 \pm 1.3$ & $85.0 \pm 0.2$ & $58.1 \pm 0.5$  \\
 \hline
       backward  &      $86.7 \pm 0.0$ & $\bm{85.3 \pm 0.3}$ & $\bm{54.0 \pm 1.7}$ & $\bm{85.7 \pm 0.1}$ & $\bm{82.1 \pm 0.1}$  \\
       backward $\hat{T}$  &      $87.0 \pm 0.0$ & $\bm{85.1 \pm 0.4}$ & $52.6 \pm 0.7$ & $\bm{85.8 \pm 0.2}$ & $\bm{77.0 \pm 1.4}$  \\
       forward  &      $86.7 \pm 0.0$ & $\bm{85.3 \pm 0.2}$ & $\bm{54.8 \pm 2.1}$ & $\bm{85.9 \pm 0.1}$ & $\bm{80.9 \pm 1.3}$  \\
       forward $\hat{T}$   &      $87.0 \pm 0.0$ & $\bm{85.2 \pm 0.3}$ & $\bm{54.7 \pm 1.7}$ & $\bm{85.9 \pm 0.2}$ & $73.0 \pm 1.2$ \\
 \hline
       unhinged (BN) &     $83.3 \pm 0.0$ & $76.9 \pm 0.5$ & $54.5 \pm 0.4$ & $80.6 \pm 0.3$ & $72.9 \pm 0.4$  \\
       sigmoid (BN)  &      $84.3 \pm 0.0$ & $80.2 \pm 0.3$ & $\bm{55.3 \pm 0.6}$ & $81.7 \pm 0.5$ & $72.8 \pm 0.6$  \\
       savage  &      $86.5 \pm 0.0$ & $84.3 \pm 0.4$ & $51.3 \pm 0.6$ & $85.2 \pm 0.3$ & $58.3 \pm 1.0$  \\
       bootstrap soft  &      $86.7 \pm 0.0$ & $84.5 \pm 0.1$ & $52.5 \pm 1.4$ & $85.1 \pm 0.1$ & $57.8 \pm 0.7$  \\
       bootstrap hard  &      $86.7 \pm 0.0$ & $84.6 \pm 0.3$ & $52.4 \pm 0.8$ & $85.1 \pm 0.3$ & $59.0 \pm 0.6$  \\
\midrule
\multicolumn{6}{c}{IMDB, word embedding + LSTM} \\
\midrule
 & \textsc{no noise}& \textsc{mild symm.} & \textsc{high symm.} & \textsc{mild asymm.} & \textsc{high asymm.} \\
 & & $N=0.1$ & $N=0.4$ & $N=0.1$ &  $N=0.4$ \\
\midrule
 \hline
 cross-entropy &      $87.8 \pm 0.4$ & $\bm{85.2 \pm 0.5}$& $\bm{58.4 \pm 3.4}$ & $86.8 \pm 0.4$ & $71.4 \pm 1.3$  \\
 \hline
       backward  &      $87.6 \pm 0.2$ & $\bm{84.3 \pm 0.9}$ & $\bm{58.9 \pm 7.4}$ & $86.7 \pm 0.5$ & $\bm{83.6 \pm 1.4}$  \\
       backward $\hat{T}$  & $87.2 \pm 0.7$&  $\bm{82.8 \pm 2.7}$ & $\bm{59.6 \pm 5.3}$ & $\bm{87.3 \pm 0.1}$ & $\bm{82.3 \pm 1.7}$\\
       forward  &      $87.5 \pm 0.2$ & $\bm{85.0 \pm 0.2}$ & $\bm{62.2 \pm 2.0}$ & $87.0 \pm 0.4$ & $\bm{84.7 \pm 0.6}$  \\
       forward $\hat{T}$   & $87.8 \pm 1.5$  & $\bm{84.1 \pm 1.0}$ & $\bm{61.6 \pm 7.0}$ & $\bm{87.5 \pm 0.2}$ & $\bm{84.2 \pm 0.9}$\\
 \hline
       unhinged (BN) &     $84.3 \pm 4.4$ & $\:\: 69.7 \pm 15.9$  & $54.1 \pm 5.0$ &  $85.2 \pm 1.2$ & $\:\: 59.4 \pm 12.9$  \\
       sigmoid (BN) & $87.7 \pm 0.5$ & $\:\: 77.6 \pm 13.6$ & $50.9 \pm 1.2$ & $\bm{86.3 \pm 3.1}$ & $\:\: \bm{70.0 \pm 14.6}$\\
       savage  &      $87.4 \pm 0.3$ & $\bm{85.1 \pm 0.6}$  & $\bm{63.9 \pm 1.8}$ & $\bm{87.2 \pm 0.3}$ & $70.4 \pm 3.8$  \\
       bootstrap soft  &      $87.1 \pm 0.6$ & $\bm{83.5 \pm 2.5}$  & $58.8 \pm 2.9$ & $\bm{86.1 \pm 1.2}$ & $69.0 \pm 5.3$  \\
       bootstrap hard  &      $86.5 \pm 0.5$ & $\bm{84.3 \pm 1.0}$  & $54.0 \pm 2.6$ & $86.7 \pm 0.4$ & $71.8 \pm 3.3$  \\
\midrule
\multicolumn{6}{c}{CIFAR10, 14-layer ResNet} \\
\midrule
 & \textsc{no noise}& \textsc{mild symm.} & \textsc{high symm.} & \textsc{mild asymm.} & \textsc{high asymm.} \\
 & & $N=0.2$ & $N=0.6$ & $N=0.2$ &  $N=0.6$ \\
\midrule
 \hline
 cross-entropy &      $87.8$ & $83.7$ & $\bm{71.7}$ & $85.0$ & $57.6$  \\
 \hline
       backward   &      $87.6$ & $81.5$ & $61.3$ & $83.8$ & $\bm{75.2}$  \\
       backward $\hat{T}$  & $87.7$ & $80.4$ & $29.7$ & $83.8$ & $66.7$\\
       forward &      $87.8$ & $\bm{85.6}$ & $\bm{75.2}$ & $86.3$ & $\bm{84.5}$  \\
       forward $\hat{T}$   & $87.4$  & $83.4$  & $65.4$ & $\bm{87.0}$ & $\bm{74.8}$ \\
 \hline
       unhinged (BN) &$86.9$ & $\bm{84.1}$ & $70.0$  & $83.8$ & $52.1$ \\
       sigmoid (BN)  & $76.0$ & $66.6$ & $51.1$ & $71.8$ & $57.0$\\
       savage  &      $80.1$ & $77.4$   & $66.7$ & $76.0$ & $50.5$  \\
       bootstrap soft  &      $87.7$ & $\bm{84.3}$  & $\bm{71.7}$ & $84.6$ & $57.8$  \\
       bootstrap hard  &      $87.3$ & $83.6$  & $\bm{71.7}$ & $84.7$ & $58.3$  \\
\midrule
\multicolumn{6}{c}{CIFAR10, 32-layer ResNet} \\
\midrule
 & \textsc{no noise}& \textsc{mild symm.} & \textsc{high symm.} & \textsc{mild asymm.} & \textsc{high asymm.} \\
 & & $N=0.2$ & $N=0.6$ & $N=0.2$ &  $N=0.6$ \\
\midrule
 \hline
 cross-entropy & $90.1$ & $86.6$  & $75.4$ & $89.0$ & $53.6$ \\
 \hline
       forward & $91.2$ & $\bm{87.7}$ & $\bm{79.1}$ & $\bm{89.9}$ & $\bm{87.6}$ \\
       forward $\hat{T}$ & $90.5$ & $\bm{87.9}$ & $75.1$ &  $\bm{90.1}$ & $\bm{77.6}$\\
       backward  & $90.1$ & $83.0$ & $62.1$ & $84.4$ & $74.3$  \\
       backward $\hat{T}$  &$90.8$ & $86.9$ & $51.4$ & $86.4$ & $66.7$ \\
 \hline
       unhinged (BN)  & $90.2$ & $86.5$ & $68.6$ & $87.1$ & $60.0$\\
       sigmoid (BN)  & $81.6$ & $69.6$ & $53.4$ & $79.1$ & $61.8$ \\
       savage & $88.3$ & $86.2$ & $73.4$ & $86.3$ & $53.5$\\
       bootstrap soft  & $90.9$ & $86.9$  & $\bm{76.3}$ & $88.6$ & $53.1$ \\
       bootstrap hard  &   $90.4$ & $86.4$  & $\bm{76.1}$ & $88.6$  & $54.7$\\
\midrule
\multicolumn{6}{c}{CIFAR100, 44-layer ResNet} \\
\midrule
 & \textsc{no noise}& \textsc{mild symm.} & \textsc{high symm.} & \textsc{mild asymm.} & \textsc{high asymm.} \\
 & & $N=0.2$ & $N=0.6$ & $N=0.2$ &  $N=0.6$ \\
\midrule
 \hline
 cross-entropy   & $68.5$ & $57.9$  & $37.7$ & $63.5$ & $17.1$ \\
 \hline
       backward   & $68.5$ & $55.1$ & $29.3$ & $53.8$ & $\bm{36.8}$ \\
       backward $\hat{T}$    & $1.0$ & $1.0$ & $1.0$ & $1.0$ & $1.0$ \\
       forward   & $68.8$ & $\bm{64.0}$ & $\bm{50.4}$ & $\bm{68.1}$ & $\bm{68.4}$ \\
       forward $\hat{T}$   & $10.0$ & $12.3$ & $8.8$ & $8.0$ & $9.0$ \\
 \hline
       unhinged (BN)  & $50.9$ & $47.5$ & $\bm{38.3}$ & $48.0$ & $14.5$\\
       sigmoid (BN)    & $58.2$ & $47.6$  & $19.2$ & $55.6$ & $16.4$ \\
       savage & $1.4$ & $2.0$ & $2.0$ & $1.8$ & $1.6$\\
       bootstrap soft  & $67.9$ & $\bm{57.8}$ & $37.4$ & $\bm{63.8}$ & $16.3$ \\
       bootstrap hard & $68.5$ & $\bm{57.3}$ & $37.8$ & $\bm{63.9}$& $\bm{17.0}$\\
\bottomrule
\end{tabular}
\caption{Numbers in bold face are mean accuracies which are statistically different form the others, by means of passing a \emph{Welch's t-test} with $5\%$ $p$-value; in case the highest accuracy is due to $\ellRobustScalar$ or $\ellFbScalar$, we highlight the next highest accuracy. For experiments without any variance information, the same rule is applied but bold face is given to the all accuracies in the range of $.5\%$ from the highest.}
\label{table:big}
\end{table*}

